Autonomous Workflow for Multimodal Fine-Grained Training Assistants Towards Mixed Reality

Autonomous artificial intelligence (AI) agents have emerged as promising protocols for automatically understanding the language-based environment, particularly with the exponential development of large language models (LLMs). However, a fine-grained, comprehensive understanding of multimodal environments remains under-explored. This work designs an autonomous workflow tailored for integrating AI agents seamlessly into extended reality (XR) applications for fine-grained training. We present a demonstration of a multimodal fine-grained training assistant for LEGO brick assembly in a pilot XR environment. Specifically, we design a cerebral language agent that integrates LLM with memory, planning, and interaction with XR tools and a vision-language agent, enabling agents to decide their actions based on past experiences. Furthermore, we introduce LEGO-MRTA, a multimodal fine-grained assembly dialogue dataset synthesized automatically in the workflow served by a commercial LLM. This dataset comprises multimodal instruction manuals, conversations, XR responses, and vision question answering. Last, we present several prevailing open-resource LLMs as benchmarks, assessing their performance with and without fine-tuning on the proposed dataset. We anticipate that the broader impact of this workflow will advance the development of smarter assistants for seamless user interaction in XR environments, fostering research in both AI and HCI communities.

==> vox.tex <==
\section{Use Case in VOXreality}
\label{sec:appendix}

\subsection{Training Assistant}
This use case aims to provide a guided AR industrial training scenario. In this use case, a trainee will work on an assembly task through interaction with 3D virtual content superimposed on the real world. During this AR assembly task, users will be guided and supported by a virtual assistant. Users will verbally engage with the virtual assistant who will be able to provide support when prompted and/or offer support when elicited based on trainee performance in the task. The AR assembly task here will involve the visualization of a holographic computer-aided-design (CAD) file. This holographic CAD file object will be interactable and composed of multiple parts which need to be assembled together by the trainee. Physical manipulation (e.g., picking up, moving, and inserting) of specific object components will be used to assemble these constituent parts into the object’s frame. Different levels of training will be offered, ranging from easy to difficult, and assembly levels can be performed in repetition. The virtual assistant will provide a unique language-centric interface with the AR training environment and aid end-user trainees in industrial assembly instruction.
\subsubsection{Scenario}
This training use case scenario will focus on the experience of a single user participating in the AR training environment. In this scenario, a user will be provided with a HoloLens 2 (and/or an android) AR smart glass device. The user will engage with the training experience as detailed below in the user journey walkthrough, but in general are predicted to consist of running through the individual difficulty levels at least one time each. The use case is currently envisioned to take approximately around 3 hours (for one person), which includes time for set-up, introduction to the hardware device, training application scenarios, clean-up, and feedback assessment periods.

The tentative predicted user journey walkthrough will in general occur with the following assumptions: 1) Only one user will be in the AR training session at a time. 2) Trainees will be inexperienced in using the HoloLens 2, and 3) Trainees will be relatively inexperienced in the industrial assembly task (i.e., unfamiliar with the CAD file to be assembled).

A user will first be introduced to the HoloLens 2 and provided an explanation of what will be happening during their AR training experience. They will then be provided with relevant consent forms to sign, and after signing they will be fitted with the HoloLens 2 and the training scenario will begin. 

After launching the application, either by a VOXReality researcher or the participant verbally with the virtual assistant, the user will be greeted by the virtual assistant and prompted to confirm they would like to begin training. After confirming, the user will then be asked by the virtual assistant which difficulty level they would like to be trained on. Following a verbal decision by the user, the training will begin. Users will then be able to see a holographic 3D industrial CAD file object which is to be assembled. This object will not be superimposed over a physical twin object in real life, but rather existing over the local surrounding environment. This object is composed of a certain number of parts which are loaded initially external to a core frame. The constituent parts are then to be picked up and inserted in the correct spatial position into the object’s frame. Depending on the difficulty level, the parts may be visually ordered in a sequential fashion or have a corresponding color-coded deposit location on the object frame. A user would then begin moving the holographic parts in space and attempting to position them into the frame. Throughout this process, the virtual assistant will be readily available to respond to help inquiries and offer support. Support is predicted to come in the form of e.g., documentation such as images or PDFs. As users pick and move the individual assembly parts into the frame, relevant UI elements are predicted to provide information which may aid in the assembly process or provide feedback on how they are performing, which could scale depending on the difficulty level selected. The virtual assistant will also monitor a users’ process and intervene when the user appears to need help. For example, if a user is attempting to insert a part in a wrong location or takes a long period of time to move forward with the assembly, the virtual assistant could engage verbally with the user and offer support.

This process is intended to continue iteratively until all constituent parts of the CAD object are assembled. The user will have learned how to assemble this object and have an understanding of the assembly process. The virtual assistant would then be able to offer the user the opportunity to restart the training again along with the option to choose a different, likely more challenging, difficulty level. The user would then be expected to try the different difficulty levels in sequence. This serial assembly practice and continued help/assistance with the virtual assistant will, in the end, have provided a unique training environment for the user. Following the completion of each difficulty level, it would be beneficial if the user could be provided with metrics associated with their performance (e.g., time spent doing the entire task, per each step, etc.) in some format. After the final difficulty level is reached, the user will end the training session by instruction to the virtual assistant. The user would then remove the HoloLens 2 and the session would be closed. Following, users will be provided with paper assessment forms to get feedback on their experience as well as discuss with VOXReality experimenters on site.

\subsubsection{Technologies}
The specific technologies intended to be utilized in this use case consist of hardware devices, which include the HoloLens 2, and likely a PC laptop where the AR assembly application will run. This application will be based in Unity and will incorporate Holo-Light’s Interactive Streaming for Augmented Reality (ISAR) SDK. ISAR-enabled applications provide a client-server environment which offloads the computationally heavy rendering process from the AR device to a dedicated server environment (e.g., laptop) with a high-quality graphics processing unit and streams the application. ISAR allows the streaming of this entire application to the HoloLens 2, which itself has an ISAR-client application installed, which permits high resolution AR visualizations with low latency. This application will further make use of Holo-Light’s Augmented Reality Engineering Space (AR3S), which will provide the basis for visualization and interaction of 3D CAD files for the assembly training tasks. The application developed for this use case, which combines both the ISAR streaming functionality and the AR training and assembly features of AR 3S will be bolstered by the virtual assistant which will be described below.

The use case will utilize the ASR component developed by the consortium to generate textual counterparts of the speech of users interacting with a digital assistant. The textual information acquired from ASR will be utilized in the DA component where a dialogue system helps the users to assemble a machine. DA component will facilitate a dialogue between the user and the corresponding assembly instructions and descriptions generated by VL component using English as a mediation language. The response generated from DA will be in English and off-the-shelf text to speech tools are envisioned to be utilized to generate an audio response.

Moreover, the agent will be composed of a NLU model that will understand what the user is talking about as well as a NLG model, that generates meaningful responses. The agent will make use of manual as an unstructured textual document that guides the agent in interacting with users. The agent will be able to display pdf, corresponding videos, or specific files, if it is asked by the user.

\subsubsection{Equipment}
As mentioned above, this use case will make use of the HoloLens 2 as the AR device of choice that the end user (trainee) will utilize to interact in the AR training environment. In addition to allowing holographic visualizations of the 3D CAD data, the HoloLens 2 possesses a microphone and speaker, enabling a full audio experience and thus leverages the ASR component, NLU, and NLG models in order to have a dynamic language experience with the virtual assistant during the training sessions. As mentioned above, a PC laptop will likely be used to host the server-side AR application which will be streamed directly to the HoloLens 2. No additional equipment is envisioned to be necessary for this use case as all interactions within the training environment occur with virtual holographic content and audio information.

\subsubsection{External Context}
Beyond the holographic CAD file objects that users will interact with in this use case, external context will include support materials which the virtual assistant will provide/offer to the user when engaging with the training session. Such content will likely consist of different images of the CAD object and its constituent parts that the user could view. Additionally, instruction manuals may also be offered in the form of PDFs which the user could view and read at their discretion. While not guaranteed to be present, a further external factor which would be beneficial to have would be videos which can show an individual part being assembled in AR space. Such factors are envisioned to be incorporated into the AR application stream which would allow the user to visualize them during the training session. Given that the entirety of the session will be occurring in AR, the external environment having a defined location is not essential for this use case. However, an ideal location would be an industrial shop floor or similar location which would approximate a canonical environment where a typical user would engage in such training.

\subsubsection{Assessment Protocol}
Following the training session, users would be asked to participate in a feedback session designed to collect information on their experiences with assembly training with emphasis on interaction with the virtual assistant. Participants will be asked to complete a questionnaire/survey and/or provide direct verbal feedback to VOXReality experimenters about the quality of their experience either verbally or by questionnaire. The results from user profiling will provide insights into what went well, what could be better, and overall impressions of the use case and its technology provided. In addition, assessment protocols are envisioned to be application metrics which are profiled during the training sessions such as e.g., time spent doing a virtual task, number of incorrect steps taken, number of times the virtual assistant had to intercede and offer help due to the latter, etc. This data can be used to scientifically approximate the efficacy of the training experience over sessions with increasing difficulty. This data will be collected from the application itself.

This assessment protocol is intended to be acquired from 3-5 users; more would be ideal if possible. Despite such a presumptive low sample size however, a robust coverage of all possible end user demographics is a goal of this use case. In particular, equal numbers of all genders will be aimed for. Language of operation will likely be in English. Users are envisioned to be readily open to technology, with little experience in XR technologies and some experience in industrial tasks.

\subsubsection{Target Population}
Target populations in this use case will be users who have a desire to work with virtual assistants for task performance during industrial assembly training. Ideal participants would be those who have no prior knowledge of the task to be performed in this use case, and those who have not had much experience with AR, so they can be instructed without prior influence biasing the training scenario. Users will likely be factory workers with some assembly experience and knowledge of assembly training in general.

